MOReL : Model-Based Offline Reinforcement Learning

In offline reinforcement learning (RL), the goal is to learn a highly rewarding policy based solely on a dataset of historical interactions with the environment. The ability to train RL policies offline can greatly expand the applicability of RL, its data efficiency, and its experimental velocity. Prior work in offline RL has been confined almost exclusively to model-free RL approaches. In this work, we present MOReL, an algorithmic framework for model-based offline RL. This framework consists of two steps: (a) learning a pessimistic MDP (P-MDP) using the offline dataset; and (b) learning a near-optimal policy in this P-MDP. The learned P-MDP has the property that for any policy, the performance in the real environment is approximately lower-bounded by the performance in the P-MDP. This enables it to serve as a good surrogate for purposes of policy evaluation and learning, and overcome common pitfalls of model-based RL like model exploitation. Theoretically, we show that MOReL is minimax optimal (up to log factors) for offline RL. Through experiments, we show that MOReL matches or exceeds state-of-the-art results in widely studied offline RL benchmarks. Moreover, the modular design of MOReL enables future advances in its components (e.g. generative modeling, uncertainty estimation, planning etc.) to directly translate into advances for offline RL.

==> ablationStudy.tex <==
\clearpage

\textbf{Importance of Pessimistic MDP} 
\label{ssec:ablation}
To highlight the importance of P-MDP, we again consider the \texttt{Pure-partial} dataset outlined above. We compare~\fname~with a nai\"ve MBRL approach that first learns a dynamics model using the offline data, followed by running model-based NPG without any safeguards against model inaccuracy. The results are summarized in Figure~\ref{fig:morel_vs_naive}. We observe that the nai\"ve MBRL approach already works well, achieving results comparable to prior algorithms like BCQ and BEAR. However,~\fname~clearly exhibits more stable and monotonic learning progress. This is particularly evident in \hopper,~\hc, and \walker, where an uncoordinated set of actions can result in the agent falling over. Furthermore, in the case of nai\"ve MBRL, we observe that performance can quickly degrade after a few hundred steps of policy improvement, such as in case of \hopper,~\hc~and~\walker. This suggests that the learned model is being over-exploited. In contrast, with~\fname, we observe that the learning curve is stable and nearly monotonic even after many steps of policy improvement. 
\begin{figure}[t!]
	\includegraphics[width=\textwidth]{figures/morel_vs_naive.pdf}
	\caption{\fname~and Naive MBRL learning curves. The x-axis plots the number of model-based NPG iterations, while y axis plots the return (value) in the real environment. The naive MBRL algorithm is highly unstable while~\fname~leads to stable and near-monotonic learning. Notice however that even naive MBRL learns a policy that performs often as well as the best model-free offline RL algorithms.}
	\label{fig:morel_vs_naive} 
\end{figure}


\textbf{Transfer from P-MDP to environment} \\[0.2cm]
Finally, we study how the learning progress in P-MDP relates to the progress in the environment. Our theoretical results (Theorem~1) suggest that the value of a policy in the P-MDP cannot substantially exceed the value in the environment. This makes the value in the P-MDP an approximate lower bound on the true performance, and a good surrogate for optimization.  In Figure~\ref{fig:pessimism_lowerbound}, we plot the value (return) of the policy in the P-MDP and environment over the course of learning. Note that the policy is being learned in the P-MDP, and as a result we observe a clear monotonic learning curve for value in the P-MDP, consistent with the monotonic improvement theory of policy gradient methods~\cite{Kakade2002CPI, SchulmanTRPO}. We observe that the value in the true environment closely correlates with the value in P-MDP. In particular, the P-MDP value never substantially exceeds the true performance, suggesting that the pessimism helps to avoid model exploitation.


\begin{figure}[t!]
	\includegraphics[width=\textwidth]{figures/morel_env_vs_sim.pdf}
	\caption{Learning curve using the \texttt{Pure-partial} dataset, see paper text for details. The policy is learned using the pessimistic MDP (P-MDP), and we plot the performance in both the P-MDP and the real environment over the course of learning. We observe that the performance in the P-MDP closely tracks the true performance and never substantially exceeds it, as predicted in section~\ref{ssec:theory}. This shows that the policy value in the P-MDP serves as a good surrogate for the purposes of offline policy evaluation and learning.}
	\label{fig:pessimism_lowerbound} 
\end{figure}



